A Many-core Machine Model for Designing Algorithms with Minimum Parallelism Overheads

We present a model of multithreaded computation, combining fork-join and single-instruction-multiple-data parallelisms, with an emphasis on estimating parallelism overheads of programs written for modern many-core architectures. We establish a Graham-Brent theorem for this model so as to estimate execution time of programs running on a given number of streaming multiprocessors. We evaluate the benefits of our model with four fundamental algorithms from scientific computing. In each case, our model is used to minimize parallelism overheads by determining an appropriate value range for a given program parameter; moreover experimentation confirms the model's prediction.

==> preliminaries.tex <==
\subsection{Elements of Syntax}
Each polynomial (for example $b$) is represented by
a coefficient array (lets, $b[0,\ldots,\deg(b)]$). 
The length of the array is 
the length of the polynomial (for $b$ it is $\deg(b) +1$).
The elements in the array are in order. For example,
$b[\deg(b)]$ is the leading coefficient.

All of
our kernel has one dimensional threads, and thread blocks.
Each thread, 
has a local variable $j$ which is defined as the {\em rank}
of the thread over all the threads in all thread blocks. 
It is computed as $t+${\sf blockID}$\times\ell$, where $t$ and
$\ell$ are the thread id and the number of threads in a thread block
respectively. In this paper, we will represent rank and thread id by
$j$ and $t$ respectively.

We launch a kernel by the following format:
{\sf kernelName}$\lll c, \ell \ggg (p_0,\ldots, p_{n-1})$.
Here, $\ell$ and $c$ are the threads number in a thread block
and the thread blocks number respectively.
{\sf kernelName} is the name of our kernel.
$(p_0,\ldots, p_{n-1})$ are the parameters for this kernel.

%{\bf sync} is a way to synchronize among threads in a
%thread block. All threads in the same block wait until
%all of them reach to that execution point.

%{\bf ThreadSynchronize()} is a function that ensures that 
%all kernel calls that have already called
%are completed before proceeding further.


==> relatedWork.tex <==
\subsection{Related Work}

We want a model that covers all 
the high level characteristics 
of a GPU. It should be simple 
in the sense
that any algorithm can be analyzed
on this model without knowing or considering
the low level execution details.  
It should be general in the sense
that our analysis of an algorithm
should not depend on any particular 
GPU or any special property of it or
the programming language syntax.
The model should estimate the complexity of an algorithm
correctly. By correctly, we mean if any algorithm
has better estimate than another algorithm, then
the first algorithm should run faster than the other
in real world. It should be able to classify any algorithm
into complexity classes. 
The purpose of this model is not to 
guide programmers in writing code in details. We believe 
this is too details and application specific. There exist
a number of ways to do so~\cite{RRSBUSH2008,YO2011,MC2012,HK2009,WMS2007}.



%models are details. not simple. not general. appropriate for a class of problem.
%no model consider all parameters.
%models could be use to predict the real computational time.
%guide the programmer to optimize the code and select the parameters.

%models can not category a problem: memory intensive,
%computational intensive.
%no exact way to classify the complexity class.
%overhead count. speed up factor.
%In one word, models are too close to real gpu card
%which is changing.

In~\cite{RRSBUSH2008}: identifies five major 
optimization categories.
The performance of
an implementation rely on each of these 
optimization technique heavily. 
It is 
assumed that memory bandwidth 
is not the primary bottleneck.  
The authors use Pareto-optimal curves to prune the  
optimization space. 


In~\cite{Che:2008:PSG:1412749.1412827}: 
some problems like
traffic simulation, thermal simulation, and k-means 
are solved on GPU and computational time is accelerated 
compare to CPU time.

In~\cite{YO2011}: 
propose a model that can
predict the performance of 
a parallel program on GPU. 
The author first 
creates microbenchmarks then they 
identify three factors:
instruction 
pipeline, local memory access and
global memory access.
Their model based on these components
successfully guide optimizations
of three real world applications.


In~\cite{MC2012}:
The paper considers some practical factors like
the number of concurrent
thread blocks which may not be optimal
due to the resource constraints.
Another similar factor is considered that is the number of threads in a thread block.
When the number of threads
are not multiple of warp size.
As the authors consider only memory intensive applications,
the working set size is also considered. If this size fits into on chip memory,
we can observe the minimum overhead in accessing memory.
Their model has  binary variables 
for each of these factors which are turned on
 if the corresponding factor is in favor of peak performance.
Otherwise overheads are computed for each category and multiplied  with the estimated running time.

 It represent both application
and model by a number of parameters.
The application is characterized by
its size, memory requirement at all levels etc.
This model shows how each parameter effect
others on real  GPU and also suggest how 
programmers can tune the parameters to observe
good performance by  real world applications.


In~\cite{HK2009}: it is suitable also for memory intensive 
problems. It measures two quantities: 
the number of memory requests and warps executed
while one warp is waiting for a memory service.

In~\cite{WMS2007}: 
propose a performance model that
can predict the performance for a given problem on GPU.
Identify factors.
This model classify problems/ subproblems into three categories:
data-linear, data-constant,
computation-dependent.


% no \IEEEPARstart
%This demo file is intended to serve as a ``starter file''
%for IEEE conference papers produced under \LaTeX\ using
%IEEEtran.cls version 1.7 and later.

%All manuscripts must be in English. These guidelines include complete descriptions of the fonts, spacing, and related information for producing your proceedings manuscripts. Please follow them %and if you have any questions, direct them to the production editor in charge of your proceedings at Conference Publishing Services (CPS): Phone +1 (714) 821-8380 or Fax +1 (714) 761-1784.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)


QRQW (Queue Read Queue Write) PRAM defined in \cite{GMR1998} is a family of PRAM models which takes memory contention into account. The work is described in the traditional sense, and the time is computed by the sum of the maximum contention at each step. The estimated running time on a p-processor QRQW PRAM is $O(work/p+time)$ that can be extended via Brent's scheduling principle.

Recently, a TMM (Threaded Many-core Memory) model is presented by Lin Ma, Kunal Agrawal, Roger D. Chamberlain \cite{MAC2012} to model the important characteristics of GPU-style, many-core architectures. It estimates the running time on $P$ cores based on the effective work and span, while the effective work of an algorithm is considered as the maximum total work of that in the traditional sense and that due to memory access. Since the work due to memory access is measured by several machine parameters, i.e. time for a global memory access, coalesced granularity, and so on, TMM analysis can order algorithms from slow to fast for many different settings of those machine parameters.


